ADGym: Design Choices for Deep Anomaly Detection

Deep learning (DL) techniques have recently found success in anomaly detection (AD) across various fields such as finance, medical services, and cloud computing. However, most of the current research tends to view deep AD algorithms as a whole, without dissecting the contributions of individual design choices like loss functions and network architectures. This view tends to diminish the value of preliminary steps like data preprocessing, as more attention is given to newly designed loss functions, network architectures, and learning paradigms. In this paper, we aim to bridge this gap by asking two key questions: (i) Which design choices in deep AD methods are crucial for detecting anomalies? (ii) How can we automatically select the optimal design choices for a given AD dataset, instead of relying on generic, pre-existing solutions? To address these questions, we introduce ADGym, a platform specifically crafted for comprehensive evaluation and automatic selection of AD design elements in deep methods. Our extensive experiments reveal that relying solely on existing leading methods is not sufficient. In contrast, models developed using ADGym significantly surpass current state-of-the-art techniques.

==> Tables/AUCPR-gym-domain_copy.tex <==
% Table generated by Excel2LaTeX from sheet 'AUCPR-small-1000-meta'

\begin{table}[h!]
\footnotesize
  \centering
  \caption{{AUCPR performance rank of design choices across different domains.}}
  \scalebox{0.55}{
    % \hspace{-0.75in}
    % \centering
    \begin{tabular}{cc|cccccccccccccc}\hline
    design                & method       & Astronautics & Biology & Botany & Chemistry & Document & Finance & Healthcare & Image & Linguistics & Network & Physical & Physics & Sociology & Web  \\\hline
    aug          & GAN          & 4            & 4       & 4      & 4         & 4        & 1       & 4          & 4     & 4           & 4       & 4        & 4       & 4         & 4    \\
    aug          & Mixup        & 1            & 1       & 1      & 2         & 3        & 3       & 3          & 1     & 1           & 1       & 2        & 1       & 1         & 1    \\
    aug          & Origin       & 3            & 2       & 2      & 3         & 2        & 4       & 2          & 3     & 3           & 3       & 1        & 2       & 3         & 2    \\
    aug          & Oversampling & 2            & 3       & 3      & 1         & 1        & 2       & 1          & 2     & 2           & 2       & 3        & 3       & 2         & 3    \\
    aug          & SMOTE        & 5            & 5       & 5      & 5         & 5        & 5       & 5          & 5     & 5           & 5       & 5        & 5       & 5         & 5    \\
    na & AE           & 3            & 3       & 2      & 2         & 1        & 2       & 2          & 3     & 4           & 3       & 2        & 3       & 4         & 3    \\
    na & FTT          & 4            & 4       & 4      & 4         & 4        & 4       & 4          & 4     & 2           & 4       & 4        & 4       & 1         & 4    \\
    na & MLP          & 1            & 2       & 3      & 1         & 2        & 1       & 1          & 1     & 3           & 1       & 1        & 1       & 2         & 2    \\
    na & ResNet       & 2            & 1       & 1      & 3         & 3        & 3       & 3          & 2     & 1           & 2       & 3        & 2       & 3         & 1    \\
    af              & LeakyReLU    & 2            & 3       & 2      & 2         & 2        & 1       & 2          & 2     & 3           & 2       & 2        & 1       & 2         & 2    \\
    af              & ReLU         & 3            & 2       & 1      & 3         & 3        & 3       & 3          & 3     & 1           & 3       & 3        & 3       & 1         & 3    \\
    af              & Tanh         & 1            & 1       & 3      & 1         & 1        & 2       & 1          & 1     & 2           & 1       & 1        & 2       & 3         & 1    \\
    lf            & bce          & 4            & 4       & 3      & 3         & 2        & 5       & 4          & 3     & 3           & 5       & 1        & 2       & 3         & 3    \\
    lf            & deviation    & 1            & 3       & 2      & 1         & 4        & 6       & 2          & 1     & 1           & 3       & 2        & 3       & 2         & 2    \\
    lf            & focal        & 5            & 6       & 5      & 5         & 6        & 2       & 5          & 5     & 6           & 4       & 6        & 5       & 5         & 5    \\
    lf            & hinge        & 2            & 1       & 1      & 4         & 3        & 3       & 1          & 2     & 2           & 2       & 3        & 1       & 1         & 1    \\
    lf            & inverse      & 6            & 5       & 6      & 6         & 5        & 4       & 6          & 6     & 5           & 6       & 5        & 6       & 6         & 6    \\
    lf            & minus        & 3            & 2       & 4      & 2         & 1        & 1       & 3          & 4     & 4           & 1       & 4        & 4       & 4         & 4    \\\hline
%    optimizer\_name       & Adam         & 1            & 1       & 1      & 1         & 1        & 2       & 1          & 1     & 1           & 1       & 1        & 1       & 1         & 1    \\
%    optimizer\_name       & RMSprop      & 2            & 2       & 2      & 2         & 2        & 1       & 2          & 2     & 2           & 2       & 2        & 2       & 2         & 2    \\
%    optimizer\_name       & SGD          & 3            & 3       & 3      & 3         & 3        & 3       & 3          & 3     & 3           & 3       & 3        & 3       & 3         & 3   \\\hline
    \end{tabular}
    }
  \label{tab:AUCPR_gym_domain_copy}%
\end{table}%


==> Tables/Dataset_Description.tex <==
% Table generated by Excel2LaTeX from sheet 'AUCPR-sota'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{c}
    \end{tabular}%
  \label{tab:dataset_des}%
\end{table}%


==> abstract_openreview.tex <==
Deep learning (DL) techniques have recently found success in anomaly detection (AD) across various fields such as finance, medical services, and cloud computing. However, most of the current research tends to view deep AD algorithms as a whole, without dissecting the contributions of individual design choices like loss functions and network architectures. This view tends to diminish the value of preliminary steps like data preprocessing, as more attention is given to newly designed loss functions, network architectures, and learning paradigms. In this paper, we aim to bridge this gap by asking two key questions: (i) Which design choices in deep AD methods are crucial for detecting anomalies? (ii) How can we automatically select the optimal design choices for a given AD dataset, instead of relying on generic, pre-existing solutions? To address these questions, we introduce ADGym, a platform specifically crafted for comprehensive evaluation and automatic selection of AD design elements in deep methods. Our extensive experiments reveal that relying solely on existing leading methods is not sufficient. In contrast, models developed using ADGym significantly surpass current state-of-the-art techniques.
